Leveraging Fixed-Parameter Tractability for Robot Inspection Planning

Autonomous robotic inspection, where a robot moves through its environment and inspects points of interest, has applications in industrial settings, structural health monitoring, and medicine. Planning the paths for a robot to safely and efficiently perform such an inspection is an extremely difficult algorithmic challenge. In this work we consider an abstraction of the inspection planning problem which we term Graph Inspection. We give two exact algorithms for this problem, using dynamic programming and integer linear programming. We analyze the performance of these methods, and present multiple approaches to achieve scalability. We demonstrate significant improvement both in path weight and inspection coverage over a state-of-the-art approach on two robotics tasks in simulation, a bridge inspection task by a UAV and a surgical inspection task using a medical robot.

==> figures/greedyMDmetricMDpseudocode.tex <==
\begin{minipage}{\linewidth}
    \begin{algorithm}[H]
      $\colorset' = \col(s)$. \tcp*{Every walk collects the colors visible from $s$.}
      \While{$|\colorset'| < k + |\col(s)|$} {
        \tcp{Choose the most dissimilar color.}
        $\colorset' = \colorset' \cup \{\argmax_{c \in \colorset} \min_{c' \in \colorset'} f(c, c')$\} \\
      }
      $\colorset' = \colorset' \setminus \col(s)$ \\
      \If{\greedymd{}} {
        Return $\colorset'$.
      }
      \If{\metricmd{}} {
        $S = \kmeans(\colorset')$ \tcp*{Run \kmeans{} with initial centroids $\colorset'$.}
        $S' = \emptyset$ \\
        \For{$s \in S$} {
          \tcp{For each centroid, choose the closest color.} 
          $S' = S' \cup \{ \argmin_{c \in \colorset' \setminus S'} d(c, s) \}$ \\
        }
        Return $S'$.

      }
    \caption{\label{alg:greedymetricMD} \greedymd{} and \metricmd{}.}
    \end{algorithm}
  \end{minipage}

==> figures/ilp.tex <==
\begin{figure}[p]
  \begin{GrayBox}{}
  \begin{tikzpicture}[node distance=1cm]
      \tikzset{
          every node/.style={{anchor=south west}, text depth=0pt},
          const/.style={},
          constLabel/.style={circle,fill=gray!25,inner sep=1.2pt, scale=0.95, font={\small}},
          comment/.style={font={\footnotesize\itshape},text width=3.2cm,color=black!60},
          longcomment/.style={font={\footnotesize\itshape},text width=5cm,color=black!60},
          headline/.style={font={}},
          mult/.style={font={\small}}
      }
      \tikzmath{
          \gridlineZero = 0; 
          \gridlineNumbers = 0.4;
          \gridlineVars = \gridlineNumbers-0.05;
          \gridlineConstraint = 1;
          \gridlineObj = 2;
          \gridlineMult = 4.9;
          \gridlineLongComment = 6.2;
          \gridlineComment = 8.0;
          \y = 0; 
          \lh = 0.85;
          \debugheight = 14;
      } 

      % DEBUG: Draw gridlines
      % \draw[dashed,draw=blue!50] (\gridlineZero,0) -- (\gridlineZero,-\debugheight);
      % \draw[dashed,draw=blue!25] (\gridlineVars,0) -- (\gridlineVars,-\debugheight);
      % \draw[dashed,draw=blue!25] (\gridlineNumbers,0) -- (\gridlineNumbers,-\debugheight);
      % \draw[dashed,draw=blue!50] (\gridlineConstraint,0) -- (\gridlineConstraint,-\debugheight);
      % \draw[dashed,draw=blue!50] (\gridlineObj,0) -- (\gridlineObj,-\debugheight);
      % \draw[dashed,draw=blue!50] (\gridlineMult,0) -- (\gridlineMult,-\debugheight);
      % \draw[dashed,draw=blue!50] (\gridlineComment,0) -- (\gridlineComment,-\debugheight);

      % Variable section
      \draw (\gridlineZero, \y) node[headline] (headVars) {Variables \& Objective};

      \tikzmath{ \y = \y - .8*\lh; }
      \draw (\gridlineVars, \y) node {$x_{u,v}, x_{v,u}$};
      \draw (\gridlineConstraint, \y) node {\hspace*{7ex}$\in \{0,1\}$ \footnotesize for $uv \in E(G)$};
      \draw (\gridlineLongComment, \y) node[longcomment] {$x_{u,v}$ is $1$ iff the directed edge $uv$ is present in the solution flow. Note that $x_{u,v}$ is distinct from $x_{v,u}$.};

      \tikzmath{ \y = \y - 1.5*\lh; }
      \draw (\gridlineVars, \y) node {$y_{e,v}$};
      \draw (\gridlineConstraint, \y) node {$\geq 0$ \footnotesize for $e \!\in\! E(G), v \!\in\! e$};
      \draw (\gridlineLongComment, \y) node[longcomment] {Amount of charges the edge~$e$ emits to its endpoint~$v$.};

      \tikzmath{ \y = \y - 1.1*\lh; }
      \draw (\gridlineVars, \y) node {$z_c$};
      \draw (\gridlineConstraint, \y) node {$\in \{0,1\}$ \footnotesize for $c \in \colorset$};
      \draw (\gridlineLongComment, \y) node[longcomment] {Only used if~$t < \colorsetsize$. Value~$1$ iff color~$c$ is collected.};

      \tikzmath{ \y = \y - 1.2*\lh; }

      % Objective
      \draw (\gridlineVars, \y) node (obj) {$
             \min \!\! \sum\limits_{uv \in E(G)} \!\!\! w(u, v) (x_{u,v} + x_{v,u})
      $};    
      \draw (\gridlineLongComment,\y) node[longcomment] {Minimize weighted cost of walk.};    

      % Flow conditions section
      \tikzmath{ \y = \y - 1.5*\lh; } 
      \draw (\gridlineZero, \y) node[headline] (headflow) {Flow conditions};

      % -- constraint 1a
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] {1a};
      \draw (\gridlineConstraint,\y) node[const] {$
          \sum\limits_{u \in N(v)} x_{u,v} - x_{v,u} = 0
      $};
      \draw (\gridlineMult,\y) node[mult] {
          for every $v \in V(G)$
      };
      \draw (\gridlineComment,\y) node[comment] {Flow preservation.};    

      % -- constraint 1b
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] {1b};
      \draw (\gridlineConstraint,\y) node {$
          \sum\limits_{u \in N(s)} x_{s,u} \geq 1
      $};    
      \draw (\gridlineComment,\y) node[comment] {Outgoing flow from source~$s$.}; 


      % Charge emitting trick
      \tikzmath{ \y = \y - 1.5*\lh; } 
      \draw (\gridlineZero, \y) node[headline] (headflow) {Prohibit closed flow disjoint from~$s$};

      % -- constraint 2a
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] {2a};
      \draw (\gridlineConstraint,\y) node {$\displaystyle
          y_{uv,u} + y_{uv,v} = 2(x_{u,v} + x_{v,u})
      $};    
      \draw (\gridlineComment,\y) node[comment] {Solution edges emit charges to neighbors, unless incident to~$s$.}; 
      \tikzmath{ \y = \y - .6*\lh; } 
      \draw (\gridlineConstraint,\y) node[mult] {
          for every $uv \in E(G - s)$
      };    
   
      % -- constraint 2b
      \tikzmath{ \y = \y - 1.4*\lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] {2b};
      \draw (\gridlineConstraint,\y) node {$
          \sum\limits_{u\in N(v) \setminus \{s\}} y_{uv,v} \leq \left(2 - \frac{2}{2n-3}\right)\cdot  \! \sum\limits_{u \in N(v)} \! x_{u,v}
      $};       
      \draw (\gridlineComment,\y) node[comment] {
          Vertices can consume slightly less than two charges.
      }; 
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineConstraint,\y) node[mult] {
          for every $v \in V(G) \setminus \{s\}$
      };        


      % Count colors
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineZero, \y) node[headline] (headcol) {Count number of collected colors};

      \tikzmath{ \y = \y - .5*\lh; } % Extra spacing
      
      % -- constraint 3a
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] (rectAStart) {3a};
      \draw (\gridlineConstraint,\y) node {$
          \sum\limits_{v \in \col^{-1}(c)} \sum\limits_{u \in N(v)} x_{u,v} \geq 1
      $};    
      \draw (\gridlineMult,\y) node[mult] {
          for every $c \in C$
      };
      \draw (\gridlineComment,\y) node[comment] (rectAEnd) {
          Collect every color.
      }; 

      \begin{pgfonlayer}{bg} 
          \draw[white,thick,fill=black!5,rounded corners] ($(rectAStart.north west)+(-0.3,0.5)$)  rectangle ($(rectAEnd.south east)+(0.1,-0.4)$);

          \coordinate (temp) at (rectAStart.north -| \gridlineConstraint,0);
          \draw ($(temp)+(0,0.15)$) node[rectangle,fill=white,rounded corners,inner sep=5pt,draw=black!5,line width=1pt] {\small Case $t = |C|$};        
      \end{pgfonlayer}
      
      \tikzmath{ \y = \y - 1.1*\lh; } % Extra space below

      % -- constraint 3b
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] (rectBStart) {3b};
      \draw (\gridlineConstraint,\y) node {$
          z_c \leq \sum\limits_{v \in \col^{-1}(c)} \sum\limits_{u \in N(v)} x_{u,v} 
      $};    
      \draw (\gridlineMult,\y) node[mult] {
          for every $c \in C$
      };    
      \draw (\gridlineComment,\y) node[comment] {
          Walk must cross vertex of color~$c$ to collect~$c$.
      }; 

      \tikzmath{ \y = \y - .4*\lh; } % Some extra space

      % -- constraint 3c
      \tikzmath{ \y = \y - \lh; } 
      \draw (\gridlineNumbers,\y) node[constLabel] {3c};
      \draw (\gridlineConstraint,\y) node {$
          \sum_{c \in C} z_c \geq t
      $};     
      \draw (\gridlineComment,\y) node[comment] (rectBEnd) {
          Collect at least~$t$ colors.
      }; 

      \begin{pgfonlayer}{bg} 
          \draw[white,thick,fill=black!5,rounded corners] ($(rectBStart.north west)+(-0.3,0.5)$)  rectangle ($(rectBEnd.south east)+(0.1,-0.5)$);

          \coordinate (temp) at (rectBStart.north -| \gridlineConstraint,0);
          \draw ($(temp)+(0,0.15)$) node[rectangle,fill=white,rounded corners,inner sep=5pt,draw=black!5,line width=1pt] {\small Case $t < \colorsetsize$};
      \end{pgfonlayer}
  \end{tikzpicture}
  \end{GrayBox}
  \caption{ILP for the \textsc{Graph Inspection} problem.}\label{fig:ilp-formulation}
\end{figure}

